The Chronicles of IIBordia: Dualities, Bordisms, and the Swampland

In this work we investigate the Swampland Cobordism Conjecture in the context of type IIB string theory geometries with non-trivial duality bundle. Quite remarkably, we find that many non-trivial bordism classes with duality bundles in Mp$(2,\mathbb{Z})$, a double cover of SL$(2,\mathbb{Z})$ related to fermions, correspond to asymptotic boundaries of well-known supersymmetric F-theory backgrounds. These include $[p,q]$-7-branes, non-Higgsable clusters, S-folds, as well as various lower-dimensional generalizations. These string theoretic objects break the global symmetries associated to the non-trivial bordism groups, providing a strong test of the Cobordism Conjecture. Further including worldsheet orientation reversal promotes the duality group to the Pin$^+$ cover of GL$(2,\mathbb{Z})$. The corresponding bordism groups require a new non-supersymmetric "reflection 7-brane" and its compactifications to ensure the absence of global symmetries, thus providing an interesting prediction of the Cobordism Conjecture for non-supersymmetric type IIB backgrounds. A major component of the present work is the explicit derivation of the involved bordism groups as well as their generators, which correspond to asymptotic boundaries of explicit string theory backgrounds. The main tool is the Adams spectral sequence, to which we provide a detailed introduction. We anticipate that the same techniques can be applied in a wide variety of settings.

==> style_points.tex <==
% we have a bunch of different diagrams with colors and styles scattered across 180 pages. The goal of this file is
% to organize everything: if you want to change a color or shape, you only have to change it here.

% TODO: I (Arun) am still working on implementing this

% this is a specification of all the colors used in the diagrams in this paper
% if you want to change a color we use, change it HERE

\colorlet{color1}{BrickRed}
\colorlet{color2}{RedOrange}
\colorlet{color3}{Goldenrod!67!black}
\colorlet{color4}{Green}
\colorlet{color5}{PineGreen}
\colorlet{color6}{MidnightBlue}
\colorlet{color7}{Fuchsia}

% when there are fewer than 7 distinct colors in a diagram, we don't want to use nearby colors (e.g. use red and
% blue, rather than red and orange). The purpose of the next definitions is to choose subsets of the above colors
% to use in two-color diagrams (2color) and four-color diagrams (4color).

\colorlet{2color1}{color1}
\colorlet{2color2}{color6}

\colorlet{4color1}{color1}
\colorlet{4color2}{color4}
\colorlet{4color3}{color6}
\colorlet{4color4}{color7}

% for stuff that's "less important" or not worth drawing attention to
\colorlet{bland}{gray!60!white}


\usetikzlibrary{shapes.geometric}

\tikzset{shape1/.style=circle}
\tikzset{shape2/.style={regular polygon,regular polygon sides=3,rotate=180}}
\tikzset{shape3/.style={regular polygon,regular polygon sides=5}}
\tikzset{shape4/.style={regular polygon,regular polygon sides=3}}
\tikzset{shape5/.style=star}
\tikzset{shape6/.style=rectangle}
\tikzset{shape7/.style=diamond}

\newcommand{\shapeone}{circle}
\newcommand{\shapetwo}{regular polygon,regular polygon sides=3,rotate=180}
\newcommand{\shapethree}{regular polygon,regular polygon sides=5}
\newcommand{\shapefour}{regular polygon,regular polygon sides=3}
\newcommand{\shapefive}{star}
\newcommand{\shapesix}{rectangle}
\newcommand{\shapeseven}{diamond}

\tikzset{2shape1/.style=shape1}
\tikzset{2shape2/.style=shape6}
\tikzset{4shape1/.style=shape1}
\tikzset{4shape2/.style=shape4}
\tikzset{4shape3/.style=shape6}
\tikzset{4shape4/.style=shape7}

\newcommand{\twoshapeone}{\shapeone}
\newcommand{\twoshapetwo}{\shapesix}

\newcommand{\fourshapeone}{\shapeone}
\newcommand{\fourshapetwo}{\shapefour}
\newcommand{\fourshapethree}{\shapesix}
\newcommand{\fourshapefour}{\shapeseven}

% combining them for ease of use in spectral sequences

\tikzset{style1/.style={filldraw=color1, shape1}}
\tikzset{style2/.style={fill=color2, shape2}}
\tikzset{style3/.style={fill=color3, shape3}}
\tikzset{style4/.style={fill=color4, shape4}}
\tikzset{style5/.style={fill=color5, shape5}}
\tikzset{style6/.style={fill=color6, shape6}}
\tikzset{style7/.style={fill=color7, shape7}}

\tikzset{2style1/.style={fill=2color1, 2shape1}}
\tikzset{2style2/.style={fill=2color2, 2shape2}}

\tikzset{4style1/.style={draw=4color1, fill=4color1, 4shape1}}
\tikzset{4style2/.style={draw=4color2, fill=4color2, 4shape2}}
\tikzset{4style3/.style={draw=4color3, fill=4color3, 4shape3}}
\tikzset{4style4/.style={draw=4color4, fill=4color4, 4shape4}}

\tikzset{stylebland/.style={draw=black,fill=bland}}

\newcommand{\styleone}{color1, \shapeone}
\newcommand{\styletwo}{color2, \shapetwo}
\newcommand{\stylethree}{color3, \shapethree}
\newcommand{\stylefour}{color4, \shapefour}
\newcommand{\stylefive}{color5, \shapefive}
\newcommand{\stylesix}{color6, \shapesix}
\newcommand{\styleseven}{color7, \shapeseveb}

\newcommand{\twostyleone}{2color1, \twoshapeone}
\newcommand{\twostyletwo}{2color2, \twoshapetwo}

\newcommand{\fourstyleone}{4color1, \fourshapeone}
\newcommand{\fourstyletwo}{4color2, \fourshapetwo}
\newcommand{\fourstylethree}{4color3, \fourshapethree}
\newcommand{\fourstylefour}{4color4, \fourshapefour}

\newcommand{\stylebland}{draw=black, fill=bland}

